LeCo: Lightweight Compression via Learning Serial Correlations

Lightweight data compression is a key technique that allows column stores to exhibit superior performance for analytical queries. Despite a comprehensive study on dictionary-based encodings to approach Shannon's entropy, few prior works have systematically exploited the serial correlation in a column for compression. In this paper, we propose LeCo (i.e., Learned Compression), a framework that uses machine learning to remove the serial redundancy in a value sequence automatically to achieve an outstanding compression ratio and decompression performance simultaneously. LeCo presents a general approach to this end, making existing (ad-hoc) algorithms such as Frame-of-Reference (FOR), Delta Encoding, and Run-Length Encoding (RLE) special cases under our framework. Our microbenchmark with three synthetic and six real-world data sets shows that a prototype of LeCo achieves a Pareto improvement on both compression ratio and random access speed over the existing solutions. When integrating LeCo into widely-used applications, we observe up to 5.2x speed up in a data analytical query in the Arrow columnar execution engine and a 16% increase in RocksDB's throughput.

==> background_sketch.tex <==
\section{Statement about the Framework}
\label{sec:background_sketch}
\begin{itemize}
    \item data compression is about digging out redundancy and structures, and represent with smaller where no structure is discernible. source encoding ( memoryless means treat records iid, can have memory: depends on predecessors, having some serial information) how to extract this kind of information? the more precise, less info remains in deltas, less bits to represent. Thus, we need model and partition to identify distribution and storage format to represent remaining information.
    \item more explicit explain about leco framework
    \item MODEL: Describe data distribution. e.g.: Delta use step-function, FOR use one-value function. 
    \item PARTITION: Once a model is chosen, detect the distribution the model describes. With parameter tolerance: To what extent the distribution is distorted from the desired distribution. e.g.: RLE uses a 'single-value' model partition with a tolerance threshold of zero. (kind of anomaly detection)
    \item STORAGE: to guarantee lossless compression, need to keep record of residuals, because predictions are not precise. how to store model and deltas in each block. If want to random access, need fix length bit packing. Variable length block need to store block offset and additional index. Some store outliers aside from normal deltas. (facebook varint)
    \item fit all the existing methods into leco framework (including introducing their alg.)
    \item We fit existing compression methods into this framework. Delta(Fix + step-function + bitvector), FOR(Fix + one-value-function + bitvector), RLE(Adaptive(tolerance=0) + one-value-function + pairwise), PForDelta(Fix + NULL + outlier) Elias-Fano(Fix/Adaptive + step-function(on high bits) + (bitvector+rank-select)), Leco(Fix/Adaptive + LR + bitvector).
    
    \item The relationship between learned-compression and data mining
    By filtering and weighting out what is regarded not relevant (or 'noisy'), it aims at making better visible, what is assumed to be hidden behind the noise, and at what seems relevant with respect to the investigated objective. (ignore the influence of noise/redundancy, outliers, let the data speaks for itself, describe the true distribution more precisely)
    outliers may cause models to be distorted, resulting in large delta in some segments, bad compression rate, but with anomaly detection in data mining, we can achieve smaller overall delta, and better compression rate. \cite{faloutsos2007data}
    \item relationship between leco and learned index, as well as NLP/video compression method (but they are not lossless)
    \item semantic compression and deep compression in DeepSqueeze
    \item achieve lossless by storing the deltas.
    \item random access and some insights.
    \item Leco works on almost-sorted integer and string columns, but doesn't support arbitrary length string compression.
\end{itemize}

We studied the principle of random access and observed that there are two necessary conditions to achieve this feature. Assume in the encoding phase, each data item is mapped into several code words. Firstly, number of code words representing each record should be O(1). Secondly, indexing into each code word should take less than O(N) time, for example, there might be a rule to calculate offset of each code word.

For example, FOR and Leco use fixed-length bit packing to encode deltas, thus we can directly calculate the offset.  If any of these two rules are violated, it lose the ability to random access. For example, Delta violates (2) because it spread its information into all records before it; Elias-Fano violates (1) and add rank-select dictionary to compensate for this.
